Input-Gen: Guided Generation of Stateful Inputs for Testing, Tuning, and Training

The size and complexity of software applications is increasing at an accelerating pace. Source code repositories (along with their dependencies) require vast amounts of labor to keep them tested, maintained, and up to date. As the discipline now begins to also incorporate automatically generated programs, automation in testing and tuning is required to keep up with the pace - let alone reduce the present level of complexity. While machine learning has been used to understand and generate code in various contexts, machine learning models themselves are trained almost exclusively on static code without inputs, traces, or other execution time information. This lack of training data limits the ability of these models to understand real-world problems in software. In this work we show that inputs, like code, can be generated automatically at scale. Our generated inputs are stateful, and appear to faithfully reproduce the arbitrary data structures and system calls required to rerun a program function. By building our tool within the compiler, it both can be applied to arbitrary programming languages and architectures and can leverage static analysis and transformations for improved performance. Our approach is able to produce valid inputs, including initial memory states, for 90% of the ComPile dataset modules we explored, for a total of 21.4 million executable functions. Further, we find that a single generated input results in an average block coverage of 37%, whereas guided generation of five inputs improves it to 45%.

==> discussion.tex <==
\section{Discussion}

The traditional security model for compilers assumes that they are typically run on trusted inputs.
Within this work, not only are we running compiler tooling over a web-sourced dataset that could
potentially contain nefarious code instances, turning the traditional compiler security model on its
head, we are also \textit{executing} these untrusted inputs. While we believe that the chance of
encountering a maliciously crafted input, much less the chance of a maliciously crafted input potentially
gaining access to a system through the use of our tooling is low given the datasets that we are operating
on is quite low due to the relatively stringent selection criteria for inclusion \cite{grossman2023compile},
it is still something to consider. This is compounded by recent supply-chain attacks like the xz backdoor \cite{2024xzbackdoor}
that were able to get malicious code into trusted channels. Even though these vulnerabilities are something
that need to be considered, we currently only support creating an allow list of system supported functions
to prevent system access to malicious inputs through the standard libraries. While this will handle most cases,
we do not currently handle cases such as inline assembly, which can be used to perform malicious operations,
such as making syscalls, without needing to use system libraries. We believe that the probability of a
malicious input is sufficiently low to not be worth investing significant effort beyond common sense
efforts. The underlying dataset that we used for evaluating in this work is relatively stringently filtered,
only pulling code from places where it has been packaged, but this level of filtering is highly language
dependent. For example C/C++ exclusively come from Spack and manually curated sources, which are guaranteed
to have multiple layers of human review before inclusion, precluding most attacks. However, for other languages
like Rust and Julia, the default language package repositories are used which require no manual review and can
be published too instantly. It is easy to forsee malicious packages uploaded to these repositories. However,
we have not observed any instances of this happening, but it is known to occur, with some attacks like misspellings
being prominent past examples on repositories like PyPi. In addition to some of the curation inherently present in
the dataset, we also break most of the assumptions about how an application would typically execute with how we
instrument individual functions and run them using the generated inputs. We believe this would preclude at least
some possible attacks.



==> figures/flame.tex <==

\begin{tikzpicture}
  \begin{scope}[local bounding box=system]

  \draw[line width=3.5mm, col6] (0, 0) node[anchor=west, text=black] {entry} -- (5, 0);
  \draw[line width=3.5mm, col7] (1, 0.4) node[text=black, anchor=west] {foo} -- (2, 0.4);
  \draw[line width=3.5mm, col9!40!white] (2.5, 0.4) node[text=black, anchor=west] {bar} -- (4.5, 0.4);
  \draw[line width=3.5mm, col13!40!white] (2.8, 0.8) node[text=black, anchor=west] {baz} -- (4.3, 0.8);

  \end{scope}

\end{tikzpicture}

==> tables/BenchmarksTab.tex <==
%\begin{tabular}{m{0.1\columnwidth} m{0.2\columnwidth} m{0.2\columnwidth} m{0.2\columnwidth} m{0.1\columnwidth} m{0.1\columnwidth} m{0.1\columnwidth}}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Name} & \multirow{2}{*}{Input} &  \# Recorded & \multicolumn{2}{c}{Build Time (s)} & \multicolumn{2}{c}{Execution Time (s)} & \multicolumn{2}{c}{Record+Execution Time (s)} \\
     &  & Kernels  &P9+NVIDIA & AMD &  P9+NVIDIA & AMD & P9+NVIDIA & AMD \\
\midrule
 LULESH &
 $-s 128 -r 11 -b 1 -c 1$ &
17 &
 7 &
 6 &
  251.82 & 
 173 &
 272 &
 233.72 
 \\
  miniFE &  
 $ -nx 200 -ny 200 -nz 200$ &
 7 &
 8 &
 6.7 &
  51.12 & 
 16.63 & 
 91 &
 63.28
 \\
   OpenMC &
 XXL event simulation &
 9 &
 180 &
 158 &
  214 & 
 141 &
 525 &
260
 \\
 \bottomrule
\end{tabular}

==> tables/GPUTerms.tex <==
%\begin{tabular}{m{0.21\columnwidth} m{0.25\columnwidth} m{0.25\columnwidth}
\begin{tabular}{l l l}
\toprule
\textbf{NVIDIA} &  \textbf{AMD}       & \textbf{Vendor Agnostic}
\\ \midrule
Streaming Multiprocessor  (SM)      & Compute Unit (CU) &  Vector Processor (VP)
\\ %\midrule
Warp & Wavefront & SIMD
\\ %\midrule 
Thread Block & Workgroup & Team
Thread  \\
\bottomrule
\end{tabular}

==> tables/systems.tex <==
%\begin{tabular}{m{0.21\columnwidth} m{0.25\columnwidth} m{0.25\columnwidth}
\begin{tabular}{r|c c}
\toprule
Name &  {Power9 + NVIDIA}       & {AMD}
\\ \midrule
CPU        & IBM Power9 &  AMD Trento 
\\ %\midrule
Physical Cores      & 40 & 64
\\ %\midrule 
Main Memory   & 256 GB     & 512 GB
\\ %\midrule
GPU        & Tesla V100-SXM2       & AMD MI-250X
\\ %\midrule
Device Memory & 16 GB                     & 128 GB \\
\bottomrule
\end{tabular}
